Attribute-Guided Encryption with Facial Texture Masking

The increasingly pervasive facial recognition (FR) systems raise serious concerns about personal privacy, especially for billions of users who have publicly shared their photos on social media. Several attempts have been made to protect individuals from unauthorized FR systems utilizing adversarial attacks to generate encrypted face images to protect users from being identified by FR systems. However, existing methods suffer from poor visual quality or low attack success rates, which limit their usability in practice. In this paper, we propose Attribute Guided Encryption with Facial Texture Masking (AGE-FTM) that performs a dual manifold adversarial attack on FR systems to achieve both good visual quality and high black box attack success rates. In particular, AGE-FTM utilizes a high fidelity generative adversarial network (GAN) to generate natural on-manifold adversarial samples by modifying facial attributes, and performs the facial texture masking attack to generate imperceptible off-manifold adversarial samples. Extensive experiments on the CelebA-HQ dataset demonstrate that our proposed method produces more natural-looking encrypted images than state-of-the-art methods while achieving competitive attack performance. We further evaluate the effectiveness of AGE-FTM in the real world using a commercial FR API and validate its usefulness in practice through an user study.

==> diffusion_commands.tex <==
\usepackage{amsmath,amsfonts,bm}

\newcommand{\defeq}{\coloneqq}
\newcommand{\grad}{\nabla}
\newcommand{\Ea}[1]{\E\left[#1\right]}
\newcommand{\Eb}[2]{\E_{#1}\!\left[#2\right]}
\newcommand{\Vara}[1]{\Var\left[#1\right]}
\newcommand{\Varb}[2]{\Var_{#1}\left[#2\right]}
\newcommand{\kl}[2]{D_{\mathrm{KL}}\!\left(#1 ~ \| ~ #2\right)}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bzero}{\mathbf{0}}
\newcommand{\bone}{\mathbf{1}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bxh}{\hat{\mathbf{x}}}
\newcommand{\btheta}{{\boldsymbol{\theta}}}
\newcommand{\bphi}{{\boldsymbol{\phi}}}
\newcommand{\bepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\brho}{{\boldsymbol{\rho}}}
\newcommand{\bmu}{{\boldsymbol{\mu}}}
\newcommand{\bnu}{{\boldsymbol{\nu}}}
\newcommand{\bSigma}{{\boldsymbol{\Sigma}}}

==> float/compare_ffhq.tex <==
\begin{figure*}[t]
\centering
% \vspace{-2mm}
\setlength\tabcolsep{1pt}
% \renewcommand{\arraystretch}{0.5}
%  \setlength{\abovecaptionskip}{3pt}
% \setlength\tabrowsep{0pt}
\scalebox{1.0}{\begin{tabular}{cccc}
% \begin{subfigure}[t]{0.22\textwidth}
% \includegraphics[width=\textwidth]{figures/original/10828.png}
% \vspace{-11mm}
% \begin{flushleft}
% \small{\textcolor{blue}{\textbf{46.98}}}
% \end{flushleft}
% \vspace{-2mm}
% \end{subfigure} 
% &
% \begin{subfigure}[t]{0.22\textwidth}
% \includegraphics[width=\textwidth]{figures/TIP-IM/10828.png}
% \vspace{-11mm}
% \begin{flushleft}
% \small{\textcolor{blue}{\textbf{64.56}}}
% \end{flushleft}
% \vspace{-2mm}
% \end{subfigure} &
% % \hspace{-2mm}
% \begin{subfigure}[t]{0.22\textwidth}
% \includegraphics[width=\textwidth]{figures/AMT-GAN/10828.png}
% \vspace{-11mm}
% \begin{flushleft}
% \small{\textcolor{blue}{\textbf{49.93}}}
% \end{flushleft}
% \vspace{-2mm}
% \end{subfigure} &
% \begin{subfigure}[t]{0.22\textwidth}
% \includegraphics[width=\textwidth]{figures/PGD_attribute_mask_parsing/10828.png}
% \vspace{-11mm}
% \begin{flushleft}
% \small{\textcolor{blue}{\textbf{63.49}}}
% \end{flushleft}
% \vspace{-2mm}
% \end{subfigure} 
% \\
\begin{subfigure}[t]{0.22\textwidth}
\includegraphics[width=\textwidth]{figures/original/10967.png}
\vspace{-11mm}
\begin{flushleft}
\small{\textcolor{blue}{\textbf{33.87}}}
\end{flushleft}
\vspace{-2mm}

\end{subfigure} 
&
\begin{subfigure}[t]{0.22\textwidth}
\includegraphics[width=\textwidth]{figures/TIP-IM/10967.png}
\vspace{-11mm}
\begin{flushleft}
\small{\textcolor{blue}{\textbf{44.64}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} &
% \hspace{-2mm}
\begin{subfigure}[t]{0.22\textwidth}
\includegraphics[width=\textwidth]{figures/AMT-GAN/10967.png}
\vspace{-11mm}
\begin{flushleft}
\small{\textcolor{blue}{\textbf{42.18}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} &
\begin{subfigure}[t]{0.22\textwidth}
\includegraphics[width=\textwidth]{figures/PGD_attribute_mask_parsing/10967.png}
\vspace{-11mm}
\begin{flushleft}
\small{\textcolor{blue}{\textbf{46.32}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} 
\\
\begin{subfigure}[t]{0.22\textwidth}
\includegraphics[width=\textwidth]{figures/original/10968.png}
\vspace{-11mm}
\begin{flushleft}
\small{\textcolor{blue}{\textbf{20.38}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} 
&
\begin{subfigure}[t]{0.22\textwidth}
\includegraphics[width=\textwidth]{figures/TIP-IM/10968.png}
\vspace{-11mm}
\begin{flushleft}
\small{\textcolor{blue}{\textbf{45.87}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} &
% \hspace{-2mm}
\begin{subfigure}[t]{0.22\textwidth}
\includegraphics[width=\textwidth]{figures/AMT-GAN/10968.png}
\vspace{-11mm}
\begin{flushleft}
\small{\textcolor{blue}{\textbf{28.96}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} &
\begin{subfigure}[t]{0.22\textwidth}
\includegraphics[width=\textwidth]{figures/PGD_attribute_mask_parsing/10968.png}
\vspace{-11mm}
\begin{flushleft}
\small{\textcolor{blue}{\textbf{30.12}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} 
\\
\begin{subfigure}[t]{0.22\textwidth}
\includegraphics[width=\textwidth]{figures/original/10971.png}
\vspace{-11mm}
\begin{flushleft}
\small{{\textcolor{blue}{\textbf{47.92}}}}
\end{flushleft}
\vspace{-2mm}
\caption{Original}
\end{subfigure} &
\begin{subfigure}[t]{0.22\textwidth}
\includegraphics[width=\textwidth]{figures/TIP-IM/10971.png}
\vspace{-11mm}
\begin{flushleft}
\small{{\textcolor{blue}{\textbf{67.32}}}}
\end{flushleft}
\vspace{-2mm}
\caption{TIP-IM \cite{yang2021towards}}
\end{subfigure} &
% \hspace{-2mm}
\begin{subfigure}[t]{0.22\textwidth}
\includegraphics[width=\textwidth]{figures/AMT-GAN/10971.png}
\vspace{-11mm}
\begin{flushleft}
\small{{\textcolor{blue}{\textbf{63.65}}}}
\end{flushleft}
\vspace{-2mm}
\caption{AMT-GAN \cite{hu2022protecting}}
\end{subfigure} &
\begin{subfigure}[t]{0.22\textwidth}
\includegraphics[width=\textwidth]{figures/PGD_attribute_mask_parsing/10971.png}
\vspace{-11mm}
\begin{flushleft}
\small{{\textcolor{blue}{\textbf{69.89}}}}
\end{flushleft}
\vspace{-2mm}
\caption{AGE-FTM (ours)}
\end{subfigure} 

\end{tabular}}

\caption{Visualization of the proposed method AGE-FTM attack with other compared methods in the FFHQ dataset. The number on the left bottom corner is the face verification confidence score from a commercial FR API Face++. }
\label{fig: compare ffhq}
% \vspace{-2mm}
\end{figure*}


==> float/performance.tex <==
\begin{table}[htbp]
    \caption{Fr\'echet video distance~\cite{unterthiner2018towards} comparisons of state-of-the-art methods and ours. The compared methods are re-trained on the CLEVRER dataset (by ours) and the other datasets (from \citet{skorokhodov2021stylegan} and \citet{yu2022generating}) with their official implementation. MoCoGAN$^\dagger$ is implemented with StyleGAN2 as its backbone for the best performance.}
    \label{table:main-results}
    \centering
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{lcccccc}
    \toprule
    & MoCoGAN$^\dagger$ & MoCoGAN-HD & VideoGPT & DIGAN &StyleGAN-V & VDPM (ours) \\
    \midrule
    \textit{256-UCF101}$^{16}$ & 1821.4 & 1729.6 & 2880.6 & 1630.2 & 1431.0 & \textbf{294.7} \\
    \textit{256-SkyTimelapse}$^{16}$ & 85.88 & 164.1 & 222.7 & 83.11 & 79.52 & \textbf{57.4} \\
    \bottomrule
    \end{tabular}
    }
    \vspace{0.05in}

    \begin{subtable}{.48\textwidth}
    \centering\small
    \resizebox{1.0\linewidth}{!}{\begin{tabular}{lccc}
    \toprule
    & DIGAN & StyleGAN-V & VDPM (ours) \\ 
    \midrule
    \textit{128-TaiChi}$^{16}$ & 128.1 & 143.5 & \textbf{121.9}  \\
    \bottomrule
    \end{tabular}
    }
    \end{subtable}
    %
    \begin{subtable}{.49\textwidth}
    \centering\small
    \resizebox{1.0\linewidth}{!}{\begin{tabular}{lccc}
    \toprule
    & DIGAN & StyleGAN-V & VDPM (ours) \\ 
    \midrule
    \textit{256-CLEVRER}$^{16}$ & - & - & 87.4 \\
    \bottomrule
    \end{tabular}
    }
    \end{subtable}

\end{table}


==> float/table_ffhq.tex <==
% \begin{table*}[h!]
% \setlength\tabcolsep{3pt}
% \centering
% \small
% \scalebox{0.9}{\begin{tabular}{@{}c|cccc|ccc@{}}
% \toprule
%  & \multicolumn{4}{c|}{Black-box Attack Ability} & \multicolumn{3}{c}{Image Quality} \\
%  \midrule
%                 &  IRSE50  &  IR152  & Facenet  & Mobileface & FID ($\downarrow$) & PSNR ($\uparrow$) & SSIM ($\uparrow$)  \\
% \midrule
% Clean &4.4 & 2.5 & 1.7 &5.2  & -& -& -\\
% \midrule
% TIP-IM \cite{yang2021towards} & \cellcolor{myred}52.3&\cellcolor{myorange}27.5 &\cellcolor{myred}12.50 &\cellcolor{myred}55.1 &39.86 &\cellcolor{myred}30.59 &\cellcolor{myred}0.880 \\
% AMT-GAN \cite{hu2022protecting} &19.9 & 16.1& 3.7& 30.4&\cellcolor{myyellow}35.23 &\cellcolor{myorange}22.08 &\cellcolor{myorange}0.845 \\

% \midrule
% AGE-TMA (ours) &\cellcolor{myorange}47.7 &\cellcolor{myred}36.6 &\cellcolor{myorange}11.2 &\cellcolor{myorange}53.9 &\cellcolor{myorange}32.04 & 18.58& 0.532\\
% AGE-FTM (ours) &\cellcolor{myyellow}28.0 & \cellcolor{myyellow}27.4& \cellcolor{myyellow}11.0&\cellcolor{myyellow}34.0 & \cellcolor{myred}31.51&\cellcolor{myyellow}18.67 & \cellcolor{myyellow}0.600 \\
% \bottomrule
% \end{tabular}}
% \caption{Quantitative evaluation of the proposed method and other compared methods with FFHQ dataset.}
% \label{table:ffhq}


% \end{table*}

\begin{table}[h!]
\setlength\tabcolsep{3pt}
\centering
\small
\scalebox{0.9}{\begin{tabular}{@{}c|cccc|c@{}}
\toprule
 & \multicolumn{4}{c|}{Black-box Attack Ability} & \multicolumn{1}{c}{Image Quality} \\
 \midrule
                &  IRSE50  &  IR152  & Facenet  & Mobileface & FID ($\downarrow$)   \\
\midrule
Clean &4.4 & 2.5 & 1.7 &5.2  & -\\
\midrule
TIP-IM \cite{yang2021towards} & \cellcolor{myred}52.3&\cellcolor{myorange}27.5 &\cellcolor{myred}12.50 &\cellcolor{myred}55.1 &39.86  \\
AMT-GAN \cite{hu2022protecting} &19.9 & 16.1& 3.7& 30.4&\cellcolor{myyellow}35.23  \\

\midrule
AGE-TMA (ours) &\cellcolor{myorange}47.7 &\cellcolor{myred}36.6 &\cellcolor{myorange}11.2 &\cellcolor{myorange}53.9 &\cellcolor{myorange}32.04\\
AGE-FTM (ours) &\cellcolor{myyellow}28.0 & \cellcolor{myyellow}27.4& \cellcolor{myyellow}11.0&\cellcolor{myyellow}34.0 & \cellcolor{myred}31.51 \\
\bottomrule
\end{tabular}}
\caption{Quantitative evaluation of the proposed method and other compared methods with FFHQ dataset.}
\label{table:ffhq}


\end{table}

% \begin{table*}[t!]
% % \setlength\tabcolsep{3pt}
% \caption{Evaluation of the AGE-FTM with other methods. PSNR, SSIM, FID and ASR are evaluated with CelebA-HQ datase. ASR at FAR@$0.01$ is evaluated in a black-box setting with the targeted model Mobileface.} \label{table:Ablation studies}
% \centering
% % \small
% \scalebox{1.0}{\begin{tabular}{@{}c|ccc|ccc@{}}
% \toprule
% Method                &  $\text{PGD}$  &  $\text{TMA}$  & $\text{FTM}$  & AGE  &  $\text{AGE-TMA}$   &  $\text{AGE-FTM}$ \\
% \midrule
% PSNR ($\uparrow$) &\cellcolor{myyellow}28.76 &\cellcolor{myorange}35.12  &\cellcolor{myred}40.01 & 19.21& 19.10 & 19.17 \\
% SSIM ($\uparrow$) &\cellcolor{myyellow}0.548 &\cellcolor{myorange}0.902 &\cellcolor{myred}0.966  &0.626  &0.566 & 0.613\\
% FID ($\downarrow$) &\cellcolor{myyellow}8.04  & \cellcolor{myorange}1.33  &\cellcolor{myred} 0.19  &27.64 &27.61 &27.63\\
% ASR ($\uparrow$) &\cellcolor{myred}85.20& 38.90 &18.07 &53.00 &\cellcolor{myorange}75.00 &\cellcolor{myyellow} 58.80 \\
% \bottomrule
% \end{tabular}}
% % \vspace{-2mm}
% \end{table*}

==> float/user_study_female.tex <==
\begin{figure*}[t]
% \vspace{-2mm}
\centering
\setlength\tabcolsep{1pt}
% \renewcommand{\arraystretch}{0.5}
%  \setlength{\abovecaptionskip}{3pt}
% \setlength\tabrowsep{0pt}
\scalebox{1.0}{\begin{tabular}{ccc}
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/age-ftm/000291.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{48.51}}}
\end{flushleft}
\vspace{-2mm}

\end{subfigure} 
&
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/tipim/000291.jpg}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{58.93}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} &
% \hspace{-2mm}
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/amt-gan/000291.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{56.47}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} 
\\

\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/age-ftm/000737.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{48.51}}}
\end{flushleft}
\vspace{-2mm}

\end{subfigure} 
&
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/tipim/000737.jpg}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{58.93}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} &
% \hspace{-2mm}
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/amt-gan/000737.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{56.47}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} 
\\

\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/age-ftm/000865.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{48.51}}}
\end{flushleft}
\vspace{-2mm}

\end{subfigure} 
&
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/tipim/000865.jpg}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{58.93}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} &
% \hspace{-2mm}
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/amt-gan/000865.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{56.47}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} 
\\

\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/age-ftm/001778.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{48.51}}}
\end{flushleft}
\vspace{-2mm}

\end{subfigure} 
&
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/tipim/001778.jpg}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{58.93}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} &
% \hspace{-2mm}
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/amt-gan/001778.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{56.47}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} 
\\

\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/age-ftm/002342.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{48.51}}}
\end{flushleft}
\vspace{-2mm}
\caption{AGE-FTM (ours)}
\end{subfigure} 
&
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/tipim/002342.jpg}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{58.93}}}
\end{flushleft}
\vspace{-2mm}
\caption{TIP-IM \cite{yang2021towards}}
\end{subfigure} &
% \hspace{-2mm}
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/amt-gan/002342.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{56.47}}}
\end{flushleft}
\vspace{-2mm}
\caption{AMT-GAN \cite{hu2022protecting}}
\end{subfigure} 

\end{tabular}}

\caption{Female images used in the user study. }
\label{fig:user_female}
% \vspace{-2mm}
\end{figure*}


==> float/user_study_male.tex <==
\begin{figure*}[t]
% \vspace{-2mm}
\centering
\setlength\tabcolsep{1pt}
% \renewcommand{\arraystretch}{0.5}
%  \setlength{\abovecaptionskip}{3pt}
% \setlength\tabrowsep{0pt}
\scalebox{1.0}{\begin{tabular}{ccc}
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/age-ftm/001543.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{48.51}}}
\end{flushleft}
\vspace{-2mm}

\end{subfigure} 
&
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/tipim/001543.jpg}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{58.93}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} &
% \hspace{-2mm}
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/amt-gan/001543.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{56.47}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} 
\\

\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/age-ftm/002608.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{48.51}}}
\end{flushleft}
\vspace{-2mm}

\end{subfigure} 
&
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/tipim/002608.jpg}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{58.93}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} &
% \hspace{-2mm}
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/amt-gan/002608.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{56.47}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} 
\\

\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/age-ftm/002632.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{48.51}}}
\end{flushleft}
\vspace{-2mm}

\end{subfigure} 
&
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/tipim/002632.jpg}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{58.93}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} &
% \hspace{-2mm}
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/amt-gan/002632.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{56.47}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} 
\\

\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/age-ftm/004233.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{48.51}}}
\end{flushleft}
\vspace{-2mm}

\end{subfigure} 
&
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/tipim/004233.jpg}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{58.93}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} &
% \hspace{-2mm}
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/amt-gan/004233.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{56.47}}}
\end{flushleft}
\vspace{-2mm}
\end{subfigure} 
\\

\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/age-ftm/005569.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{48.51}}}
\end{flushleft}
\vspace{-2mm}
\caption{AGE-FTM (ours)}
\end{subfigure} 
&
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/tipim/005569.jpg}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{58.93}}}
\end{flushleft}
\vspace{-2mm}
\caption{TIP-IM \cite{yang2021towards}}
\end{subfigure} &
% \hspace{-2mm}
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/user_study/amt-gan/005569.png}
\vspace{-9mm}
\begin{flushleft}
% \small{\textcolor{white}{\textbf{56.47}}}
\end{flushleft}
\vspace{-2mm}
\caption{AMT-GAN \cite{hu2022protecting}}
\end{subfigure} 

\end{tabular}}

\caption{Male images used in the user study. }
\label{fig:user_male}
% \vspace{-2mm}
\end{figure*}

